Iterative Detection and Decoding for Cell-Free Massive Multiuser MIMO with LDPC Codes

This paper proposes an iterative detection and decoding (IDD) scheme for a cell free massive multiple input multiple output (CF-mMIMO) system. Users send coded data to the access points (APs), which is jointly detected at central processing unit (CPU). The symbols are exchanged iteratively in the form of log likelihood ratios (LLRs) between the detector and the low-density parity check codes (LPDC) decoder, increasing the coded system's performance. We propose a list-based multi-feedback diversity with successive interference cancellation (MF-SIC) to improve the performance of the CF-mMIMO. Furthermore, the proposed detector is compared with the parallel interference cancellation (PIC) and MF-PIC schemes. Finally, the bit error rate (BER) performance of CF-mMIMO is compared with the co-located mMIMO (Col-mMIMO).

==> BER_ITERATIONS.tex <==
\begin{center}
\begin{tabular}{rl}
\begin{tikzpicture}

%\pgfplotsset{every axis label/.append style={font=\footnotesize},
%every tick label/.append style={font=\footnotesize},
%every plot/.append style={ultra thick} 
%}



\begin{axis}[%
%tiny,
name=mse,
%ymode=log,
width  = 0.35\columnwidth,%5.63489583333333in,
%height = 0.3\columnwidth,%4.16838541666667in,
height = 0.35\columnwidth,%4.16838541666667in,
scale only axis,
xmin  = -5,
xmax  = 15,
xlabel= {SNR [dB]},
xmajorgrids,
ymin=0.00001,
ymax=0.1,
ymode=log,
ylabel={BER},
ymajorgrids,
legend entries={SIC-IDD $=1$,
					SIC-IDD $=2$,
               % MF-SIC,
                %PIC,
				%MF-PIC,	
				%MMSE based comparator network,				
				},
legend style={fill=white, fill opacity=0.6, draw opacity=1,
text opacity =1,at={(0.01,0.01)}, anchor= south west,draw=black,fill=white,legend cell align=left,font=\scriptsize}
]

\addlegendimage{smooth,color=red,solid, thick, mark=square,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}}
\addlegendimage{smooth,color=red,dashed, thick, mark=square,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}}
%% Ellipsoids
\addplot+[smooth,color=red,solid,thick, every mark/.append style={solid} ,mark=square,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
-5  0.030451953125	\\
0	0.01044775390625\\
5	0.00283125	\\
10	0.0005033203125	\\
15	0.00005986328125	\\
20	0.00000869140625	\\
25	0.00000205078125	\\
};
%\addlegendentry{MMSE col}


\addplot+[smooth,color=red,dashed, thick, every mark/.append style={solid} ,mark=square,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
-5	0.0256708984375	\\
0	0.00806884765625\\
5	0.0020681640625	\\
10	0.0004501953125	\\
15	0.00003984375	\\
20	0.00000224609375	\\
25	0.00000087890625	\\
};
%\addlegendentry{SIC col}
%\addlegendentry{MF PIC cf}
\addplot[smooth,color=red, thick, every mark/.append style={solid} ,mark=o,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
	-1 -2\\
};\label{P33}

\addplot[smooth,color=black,thick,dashed, every mark/.append style={solid} ,mark=triangle, 
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
	-1 -2\\
};\label{P34}

\addplot[smooth,color=red,thick,dotted, every mark/.append style={dashed} ,mark=star, 
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
	-1 -1\\
};\label{P35}



\node [draw,fill=white, fill opacity=0.6,draw opacity=1,
text opacity =1,at ={(-20,4.75)}, anchor= north west,draw=black,fill=white,font=\scriptsize]  {
\setlength{\tabcolsep}{0.5mm}
\renewcommand{\arraystretch}{.8}
\begin{tabular}{l}
\ref{P35}{\hspace{0.15cm} $N_r=10$}\\
\ref{P34}{\hspace{0.15cm} $N_r=7$}\\
\ref{P33}{\hspace{0.15cm} $N_r=4$}\\
\end{tabular}
};


\end{axis}
%\end{tikzpicture}
%\begin{tikzpicture}
%\pgfplotsset{every axis label/.append style={font=\footnotesize},
%every tick label/.append style={font=\footnotesize},
%every plot/.append style={ultra thick} 
%}

\begin{axis}[%
%tiny,
name=mse,
%ymode=log,
width  = 0.35\columnwidth,%5.63489583333333in,
%height = 0.3\columnwidth,%4.16838541666667in,
height = 0.35\columnwidth,%4.16838541666667in,
scale only axis,
xmin  = -5,
xmax  = 15,
xlabel= {SNR [dB]},
xmajorgrids,
ymin=0.00001,
ymax=0.1,
ymode=log,
ylabel={BER},
ymajorgrids,
legend entries={MF-SIC-IDD $=1$,
					MF-SIC-IDD $=2$, 
					%SIC,
                %MF-SIC,
                %PIC,
				%MF-PIC,	
				%MMSE based comparator network,				
				},
legend style={fill=white, fill opacity=0.6, draw opacity=1,
text opacity =1,at={(0.01,0.01)}, anchor= south west,draw=black,fill=white,legend cell align=left,font=\scriptsize}
]

\addlegendimage{smooth,color=red,solid, thick, mark=star,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}}
\addlegendimage{smooth,color=red,dashed, thick, mark=star,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}}
%% Ellipsoids
\addplot+[smooth,color=red,solid,thick, every mark/.append style={solid} ,mark=star,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
-5	0.0300701171875	\\
0	0.01023994140625\\
5	0.00277900390625	\\
10	0.0004951171875	\\
15	0.0000599609375	\\
20	0.00000859375	\\
25	0.00000205078125	\\
};
%\addlegendentry{MMSE col}


\addplot+[smooth,color=red,dashed, thick, every mark/.append style={dashed} ,mark=star,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
-5	0.02534306640625	\\
0	0.00751435546875\\
5	0.001775	\\
10	0.00027626953125	\\
15	0.00002451171875	\\
20	0	\\
25	0.00000107421875	\\
};
%\addlegendentry{SIC col}
%\addlegendentry{MF PIC cf}
\addplot[smooth,color=black, thick, every mark/.append style={solid} ,mark=o,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
	-1 -2\\
};\label{P33}

\addplot[smooth,color=black,thick,dashed, every mark/.append style={solid} ,mark=triangle, 
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
	-1 -2\\
};\label{P34}

\addplot[smooth,color=black,thick,dotted, every mark/.append style={solid} ,mark=square, 
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
	-1 -1\\
};\label{P35}



\node [draw,fill=white, fill opacity=0.6,draw opacity=1,
text opacity =1,at ={(-20,4.75)}, anchor= north west,draw=black,fill=white,font=\scriptsize]  {
\setlength{\tabcolsep}{0.5mm}
\renewcommand{\arraystretch}{.8}
\begin{tabular}{l}
\ref{P35}{\hspace{0.15cm} $N_r=10$}\\
\ref{P34}{\hspace{0.15cm} $N_r=7$}\\
\ref{P33}{\hspace{0.15cm} $N_r=4$}\\
\end{tabular}
};
\end{axis}
%\end{tikzpicture}
\\
%
%\begin{tikzpicture}
%\pgfplotsset{every axis label/.append style={font=\footnotesize},
%every tick label/.append style={font=\footnotesize},
%every plot/.append style={ultra thick} 
%}
\begin{axis}[%
%tiny,
name=mse,
%ymode=log,
width  = 0.35\columnwidth,%5.63489583333333in,
%height = 0.3\columnwidth,%4.16838541666667in,
height = 0.35\columnwidth,%4.16838541666667in,
scale only axis,
xmin  = -5,
xmax  = 15,
xlabel= {SNR [dB]},
xmajorgrids,
ymin=0.00001,
ymax=0.1,
ymode=log,
ylabel={BER},
ymajorgrids,
legend entries={PIC-IDD $=1$,
					PIC-IDD $=2$,
                %MF-SIC,
               % PIC,
				%MF-PIC,	
				%MMSE based comparator network,				
				},
legend style={fill=white, fill opacity=0.6, draw opacity=1,
text opacity =1,at={(0.01,0.01)}, anchor= south west,draw=black,fill=white,legend cell align=left,font=\scriptsize}
]

\addlegendimage{smooth,color=magenta,solid, thick, mark=o,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}}
\addlegendimage{smooth,color=magenta,dashed, thick, mark=o,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}}
%% Ellipsoids
\addplot+[smooth,color=magenta,solid,thick, every mark/.append style={solid} ,mark=o,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
-5	0.03062529296875	\\
0	0.0105828125\\
5	0.00287822265625	\\
10	0.00050859375	\\
15	0.000061328125	\\
20	0.00000908203125	\\
25	0.0000015625	\\
};
%\addlegendentry{MMSE col}


\addplot+[smooth,color=magenta,dashed, thick, every mark/.append style={dashed} ,mark=o,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
-5	0.01959814453125	\\
0	0.00513115234375\\
5	0.0009478515625\\
10	0.00011806640625	\\
15	0.00000869140625	\\
20	0	\\
25	0	\\
};
%\addlegendentry{SIC col}
%\addlegendentry{MF PIC cf}
\addplot[smooth,color=black, thick, every mark/.append style={solid} ,mark=o,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
	-1 -2\\
};\label{P33}

\addplot[smooth,color=black,thick,dashed, every mark/.append style={solid} ,mark=triangle, 
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
	-1 -2\\
};\label{P34}

\addplot[smooth,color=black,thick,dotted, every mark/.append style={solid} ,mark=square, 
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
	-1 -1\\
};\label{P35}



\node [draw,fill=white, fill opacity=0.6,draw opacity=1,
text opacity =1,at ={(-20,4.75)}, anchor= north west,draw=black,fill=white,font=\scriptsize] 
{
\setlength{\tabcolsep}{0.5mm}
\renewcommand{\arraystretch}{.8}
\begin{tabular}{l}
\ref{P35}{\hspace{0.15cm} $N_r=10$}\\
\ref{P34}{\hspace{0.15cm} $N_r=7$}\\
\ref{P33}{\hspace{0.15cm} $N_r=4$}\\
\end{tabular}
};


\end{axis}
\end{tikzpicture}%

%\begin{tikzpicture}[baseline,trim axis right]



%\pgfplotsset{every axis label/.append style={font=\footnotesize},
%every tick label/.append style={font=\footnotesize},
%every plot/.append style={ultra thick} 
%}




%\begin{axis}[%
%tiny,
%name=mse,
%ymode=log,
%width  = 0.35\columnwidth,%5.63489583333333in,
%height = 0.3\columnwidth,%4.16838541666667in,
%height = 0.35\columnwidth,%4.16838541666667in,
%scale only axis,
%xmin  = -5,
%xmax  = 15,
%xlabel= {SNR [dB]},
%xmajorgrids,
%ymin=0.00001,
%ymax=0.1,
%ymode=log,
%ylabel={BER},
%ymajorgrids,
%legend entries={MF-PIC-IDD $=1$,
			%	MF-PIC-IDD $=2$,
                %MF-SIC,
                %PIC,
				%MF-PIC,	
				%MMSE based comparator network,				
%				},
%legend style={fill=white, fill opacity=0.6, draw opacity=1,
%text opacity =1,at={(0.01,0.01)}, anchor= south west,draw=black,fill=white,legend cell align=left,font=\scriptsize}
%]

%\addlegendimage{smooth,color=green,solid, thick, mark=diamond,
%y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}}
%\addlegendimage{smooth,color=green,dashed, thick, mark=diamond,
%y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}}
%% Ellipsoids
%\addplot+[smooth,color=green,solid,thick, every mark/.append style={solid} ,mark=diamond,
%y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
 % table[row sep=crcr]{%
%-5	0.03062529296875	\\
%0	0.0105828125\\
%5	0.00287822265625	\\
%10	0.00050859375	\\
%15	0.000061328125	\\
%20	0.00000908203125	\\
%25	0.0000015625	\\
%};
%\addlegendentry{MMSE col}


%\addplot+[smooth,color=green,dashed, thick, every mark/.append style={dashed} ,mark=diamond,
%y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
 % table[row sep=crcr]{%
%-5	0.01959814453125	\\
%0	0.00513115234375\\
%5	0.0009478515625\\
%10	0.00011806640625	\\
%15	0.00000869140625	\\
%20	0	\\
%25	0	\\
%};
%\addlegendentry{SIC col}
%\addlegendentry{MF PIC cf}
%\addplot[smooth,color=black, thick, every mark/.append style={solid} ,mark=o,
%y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
 % table[row sep=crcr]{%
%	-1 -2\\
%};\label{P33}

%\addplot[smooth,color=black,thick,dashed, every mark/.append style={solid} ,mark=triangle, 
%y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  %table[row sep=crcr]{%
%	-1 -2\\
%};\label{P34}

%\addplot[smooth,color=black,thick,dotted, every mark/.append style={solid} ,mark=square, 
%y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  %table[row sep=crcr]{%
%	-1 -1\\
%};\label{P35}



%\node [draw,fill=white, fill opacity=0.6,draw opacity=1,
%text opacity =1,at ={(-20,4.75)}, anchor= north west,draw=black,fill=white,font=\scriptsize]  {
%\setlength{\tabcolsep}{0.5mm}
%\renewcommand{\arraystretch}{.8}
%\begin{tabular}{l}
%\ref{P35}{\hspace{0.15cm} $N_r=10$}\\
%\ref{P34}{\hspace{0.15cm} $N_r=7$}\\
%\ref{P33}{\hspace{0.15cm} $N_r=4$}\\
%\end{tabular}
%};


%\end{axis}
%\end{tikzpicture}%
\\
\end{tabular}%
\end{center}

